Unsupervised Learning on a DIET: Datum IndEx as Target Free of Self-Supervision, Reconstruction, Projector Head

Costly, noisy, and over-specialized, labels are to be set aside in favor of unsupervised learning if we hope to learn cheap, reliable, and transferable models. To that end, spectral embedding, self-supervised learning, or generative modeling have offered competitive solutions. Those methods however come with numerous challenges \textit{e.g.} estimating geodesic distances, specifying projector architectures and anti-collapse losses, or specifying decoder architectures and reconstruction losses. In contrast, we introduce a simple explainable alternative -- coined \textbf{DIET} -- to learn representations from unlabeled data, free of those challenges. \textbf{DIET} is blatantly simple: take one's favorite classification setup and use the \textbf{D}atum \textbf{I}nd\textbf{E}x as its \textbf{T}arget class, \textit{i.e. each sample is its own class}, no further changes needed. \textbf{DIET} works without a decoder/projector network, is not based on positive pairs nor reconstruction, introduces no hyper-parameters, and works out-of-the-box across datasets and architectures. Despite \textbf{DIET}'s simplicity, the learned representations are of high-quality and often on-par with the state-of-the-art \textit{e.g.} using a linear classifier on top of DIET's learned representation reaches $71.4\%$ on CIFAR100 with a Resnet101, $52.5\%$ on TinyImagenet with a Resnext50.

==> content/background_nce.tex <==
\newpage
\section{Act I: Score Matching and Noise-Contrastive Estimation Origins}
\label{sec:background}

\url{https://arxiv.org/abs/2210.00726}


\url{https://proceedings.mlr.press/v108/uehara20a.html}


separation of classes \url{https://arxiv.org/abs/1909.06930}

beyond softmax \url{https://www.sciencedirect.com/science/article/pii/S0925231220318178#b0110}

infomax\url{https://arxiv.org/pdf/1808.06670.pdf?source=post_page---------------------------}

pseudo spherical contrastive divergence \url{https://arxiv.org/pdf/2111.00780.pdf}

improved contrastive divergence \url{https://arxiv.org/pdf/2012.01316.pdf}

kernel doubly dual embedding \url{https://arxiv.org/abs/1811.02228}
\url{https://arxiv.org/abs/2209.14430}

conjugate energy based model \url{https://arxiv.org/pdf/2106.13798.pdf}

hastie 14.2.4 \url{https://hastie.su.domains/Papers/ESLII.pdf}

stat efficiency \url{http://proceedings.mlr.press/v108/uehara20a/uehara20a.pdf}
\url{https://arxiv.org/pdf/1808.07983.pdf}

infoNCE VAE \url{https://arxiv.org/pdf/2107.02495.pdf}

Given samples $\vx^{(n)} \sim p_{X}, n=1,\dots,N$ one often requires to learn a parametric density $\hat{p}_{X}(.;\theta)$ to $p_{X}$. If such density is in the form of an {\em Energy Based Model} (EBM) then it is expressed as
\begin{align}
    \hat{p}_{X}(\vx;\vtheta) \triangleq \frac{1}{Z(\vtheta)}\exp(f_{\vtheta}(\vx)),
\end{align}
with $f_{\vtheta}$ any $\sX \mapsto \mathbb{R}$ parametrized {\em energy function}; the {\em partition function} $Z(\vtheta)\triangleq\int \exp(f_{\vtheta}(\vx)) d\vx$ is considered to be intractable. We will denote the functional $\hat{p}_{X}(.;\theta)$ by $\hat{p}_{X}$ hereon.\\
{\bf Our goal} is to produce an estimate $\hat{\vtheta}$ of the model's parameters without estimating $Z(\vtheta)$ and such that $\exp(f_{\hat{\vtheta}}(\vx)) \propto p_{X}$. We will see below that the two main family of techniques that do not rely on $Z(\vtheta)$ are the Score Matching and Noise Contrastive Estimator methods.



{\bf Input space solution.}~Score Matching (SM) \citep{hyvarinen2005estimation} proposes to approximate a different functional
\begin{align*}
\vp_{X}(\vx) \propto \exp(f_{\vtheta}(\vx)),\forall \vx
&\iff 
\exists c > 0 : \vp_{X}(\vx) = c\exp(f_{\vtheta}(\vx)),\forall \vx\\
&\iff 
\exists c \in \mathbb{R} : \log(\vp_{X}(\vx)) = c+f_{\vtheta}(\vx),\forall \vx\\
&\iff \nabla_{\vx} \log(\vp_{X}(\vx)) =\nabla_{\vx}f_{\vtheta}(\vx),\forall \vx,
\end{align*}
where the first statement comes from definition of proportionality, in the second step application of the $\log$ means that the constant is not longer positive only and the statement holds by bijectivity of the $\log$ on $\mathbb{R}^+$, and the last statement comes from the fact that if two mappings are shifted versions of each other, their derivative must be equal. In short, SM proposes the following reformulation
\begin{align}
    \text{ goal } \hat{p}_{\theta} \approx p_{X} \xrightarrow{\text{SM}} \nabla_{\vx}\log(\hat{p}_{X}) \approx \nabla_{\vx}f_{\vtheta}(\vx),\label{eq:SM}
\end{align}
and thus the partition function is no longer required. We emphasize that $\nabla_{\vx}f_{\vtheta}(\vx)$ is commonly referred to as the {\em score function}; SM's loss is therefor given by
\begin{align}
\underbrace{\mathbb{E}_{\vx \sim p_{X}}\hspace{-0.1cm}\left[\frac{1}{2}\left\|\nabla_{\vx}f_{\vtheta}(\vx) -\nabla_{\vx}\log(p_{X}(\vx))\right\|_2^2\right]}_{\mathclap{\text{Explicit Score Matching (ESM)}}}\hspace{-0.1cm}=\underbrace{\mathbb{E}_{\vx \sim p_{X}}\hspace{-0.1cm}\left[\frac{1}{2}\left\|\nabla_{\vx}f_{\vtheta}(\vx) \right\|_2^2+\Tr(\Hess(f_{\vtheta})(\vx))\right]}_{\mathclap{\text{Implicit Score Matching (ISM)}}}+{\rm cst}.\label{eq:ISM}
\end{align}
The equality is worth deriving to understand the assumptions that need to hold for EMS to recover ISM and back; it relies on a simple application of the Integration By Parts (IBP) \citep{royden1988real} and the observation that $\nabla_{\vx}p_{X}(\vx)=\frac{p_{X}(\vx)}{p_{X}(\vx)}\nabla_{\vx}p_{X}(\vx)=p_{X}(\vx)\nabla_{\vx}\log(p_{X}(\vx))$ (*) leading to
\begin{align*}
    {\rm ESM}=&\mathbb{E}_{\vx \sim p_{X}}\hspace{-0.1cm}\left[\frac{1}{2}\left\|\nabla_{\vx}f_{\vtheta}(\vx) \right\|_2^2\right]-\mathbb{E}_{\vx \sim p_{X}}\hspace{-0.1cm}\left[\langle\nabla_{\vx}f_{\vtheta}(\vx),\nabla_{\vx}\log(p_{X}(\vx))\rangle \right]+{\rm cst}\\
    =&\mathbb{E}_{\vx \sim p_{X}}\hspace{-0.1cm}\left[\frac{1}{2}\left\|\nabla_{\vx}f_{\vtheta}(\vx) \right\|_2^2\right]-\int_{\sX} \langle \nabla_{\vx} f_{\vtheta}(\vx),\nabla_{\vx} p_{X}(\vx)\rangle d\vx+{\rm cst}&&\text{(*)}\\
    =&\mathbb{E}_{\vx \sim p_{X}}\hspace{-0.1cm}\left[\frac{1}{2}\left\|\nabla_{\vx}f_{\vtheta}(\vx) \right\|_2^2\right]-\sum_{d=1}^{D}\int_{\sX}  \frac{\partial  f_{\vtheta}}{\partial x_d}(\vx)\frac{\partial  p_X}{\partial x_d}(\vx) d\vx+{\rm cst}&&\text{(linearity of int.)}\\
    =&\mathbb{E}_{\vx \sim p_{X}}\hspace{-0.1cm}\left[\frac{1}{2}\left\|\nabla_{\vx}f_{\vtheta}(\vx) \right\|_2^2\right]-\sum_{d=1}^{D}\int_{\sX_{i\not = d}}\left[\frac{\partial f_{\vtheta}}{\partial x_d}(\vx)p_{X}(\vx) \right]_{x_d=-\infty}^{x_d=\infty}dx_{i \not = d} \\
    &\hspace{5cm}+\sum_{d=1}^{D}\int_{\sX} p_X(\vx)\frac{\partial^2 f_{\vtheta}}{\partial x_d^2}(\vx) d\vx+{\rm cst}&&\text{(IBP on $x_d$)}\\
    {\rm ISM}=&\mathbb{E}_{\vx \sim p_{X}}\hspace{-0.1cm}\left[\frac{1}{2}\left\|\nabla_{\vx}f_{\vtheta}(\vx) \right\|_2^2\right]-0+\mathbb{E}_{\vx \sim p_{X}}\left[\Tr(\Hess(f_{\vtheta})(\vx))\right]+{\rm cst},&&\mbox{(compact supp.)}
\end{align*}
and thus ISM removes the need to know $\nabla_{\vx}\log p_{X}$ to learn our score function $\nabla_{\vx} f_{\vtheta}$. Despite its ingenuous construction, {\em SM presents practical challenges: ESM requires an approximation of $\nabla_{\vx}\log(p_{X})$ and ISM requires computation of the Hessian's matrix diagonal, both tasks becoming increasingly difficult for high-dimensional data}.



{\bf Latent space solution.}~Noise Contrastive Estimation (NCE) proposes to set-up a binary classification problem between samples from $p_{X}$ and samples from a user-specified noise distribution $p_{\epsilon}$. Using $\log(p_{X|Y}(\vx|1))=f_{\theta}(\vx)$ and $p_{X|Y}(\vx|0)=p_{\epsilon}(\vx)$, Bayes rule leads to
\begin{align}
    p_{Y|X}(1|\vx)=\frac{p_{X|Y}(\vx|1)p_Y(1)}{p_{X|Y}(\vx|1)p_Y(1)+p_{X|Y}(\vx|0)p_Y(0)}=\sigmoid(f_{\theta}(\vx)-\log(p_{\epsilon}(\vx)\nu)),\label{eq:NCE}
\end{align}
with $\sigmoid$ the sigmoid function, and $\nu\triangleq p_Y(0)/p_Y(1)$ is the ratio of noise samples versus original samples. The loss to minimize is thus given by the negative lok-likelihood
\begin{align}
    \mathcal{L}(\vx,y)=-\1_{\{y=1\}}\log(p_{Y|X}(1|\vx))-\1_{\{y=0\}}\log(1-p_{Y|X}(1|\vx)).\label{eq:cross_entropy}
\end{align}
The remarkable property of NCE is that the energy function $\exp(f_{\theta})$ will self-normalize so that in the limit of infinite noise samples ($\nu \rightarrow \infty$), and with noise samples living on a domain that includes the data domain ($p_X(\vx)>0 \implies p_{\epsilon}(\vx)>0$), then the energy functions will converge to the data density as in $\exp(f_{\vtheta}(\vx))=p_X(\vx)$, and thus $Z(\vtheta)=1$. Despite this apparent benefit, {\em NCE presents practical challenges: it requires to define a noise distribution which greatly impact performances if not set carefully \citep{chehab2022optimal} and to densely sample the input space which becomes challenging for high-dimensional data}.




\section{Act II: Score Matching and Noise-Contrastive Estimation For High-Dimensional Data}
\label{sec:improvements}


{\bf Sliced score matching}
sliced score matching \url{http://auai.org/uai2019/proceedings/papers/204.pdf}
also equivalent to NCE with noise distribution being data plus direction vector $\vv$.
\begin{align}
\mathbb{E}_{\substack{\vx \sim p_{X}\\\vv \sim p_{V}}}\hspace{-0.1cm}\left[\frac{\left(\vv^T\nabla_{\vx}f_{\vtheta}(\vx) -\vv^T\nabla_{\vx}\log(p_{X})(\vx)\right)^2}{2}\right]\hspace{-0.1cm}=\hspace{-0.1cm}\mathbb{E}_{\substack{\vx \sim p_{X}\\\vv \sim p_{V}}}\hspace{-0.1cm}\left[\frac{\left(\vv^T\nabla_{\vx}f_{\vtheta}(\vx) \right)^2}{2}+\vv^T\Hess f_{\vtheta} (\vx)\vv\right]+{\rm cst}.\label{eq:ISM}
\end{align}

{\bf From Score Matching to Denoising Autoencoders and Diffusion Models}

Since the RHS of \cref{eq:ISM} is not tractable for high-dimensional data, \citet{vincent2011connection} introduces a {\em noise distribution} $p_{\tilde{X},X}$ to be used in-place of $p_{X}$. In particular, when a RBF kernel density estimate is used 
$$p_{\tilde{X},X}(\tilde{\vx},\vx)=\frac{1}{\sqrt{2\pi }\sigma}\exp\left(\frac{\|\tilde{\vx}-\vx\|_2^2}{2\sigma^2}\right)$$
then training consiss in sampling training set samples, adding white noise with standard deviation $\sigma$ and minimizing the following {\em Denoising Score Matching} loss
\begin{align}
\mathcal{L}_{\rm DSM}=\mathbb{E}_{(\tilde{\vx},\vx) \sim p_{\tilde{X},X}}\left[\frac{1}{2}\left\|f_{\theta}(\tilde{\vx}) -\frac{\vx-\tilde{\vx}}{\sigma_i^2}\right\|_2^2\right],
\end{align}
recovering a denoising autoencoder if the mapping is of the form $f_{\theta}(\tilde{\vx})=\frac{g_{\theta}(\vx-\tilde{\vx})}{\sigma_i^2}$. The ``one-shot denoising'' of DSM was then extended by Noise Conditional Score Networks (NCSNs) \citet{song2019generative}. In this {\em multiscale} version of DSM, a multi-stage denoising is learned via minimization of
\begin{align}
\mathcal{L}_{\rm NCSN}=\frac{1}{L}\sum_{i=1}^{L}\lambda(\sigma_i)\mathbb{E}_{(\vx,\tilde{\vx}) \sim p_{X,\tilde{X}_i}}\left[\frac{1}{2}\left\|f_{\theta}(\tilde{\vx},\sigma_i) -\frac{\vx-\tilde{\vx}}{\sigma^2_i}\right\|_2^2\right],
\end{align}
with $\lambda(\sigma_i)$ a weight function, usually taken to be $\lambda(\sigma)=\sigma^2$, and where the network's input include the scale variable $\sigma_i$.

A slight variation of ISM introduced in \citet{kingma2010regularized} adds a regularizer term $\lambda \left\| \nabla_{\vx}f_{\theta}(\vx)\right\|_2^2$. 


Variants of NCE include improvements of its loss landscape e.g. using higher-order optimizers and employing the log-loss instead of cross-entropy \citep{liu2021analyzing}.



In the same spirit as DSM extended SM, Conditional NCE (CNCE) has been introduced \citep{ceylan2018conditional} to work on a conditional distribution of the data. In short, one also defines $p_{\tilde{X},X}(\tilde{\vx},\vx)$ but now then solves the binary classification problem of $(\tilde{\vx},\vx)$ versus $(\vx,\tilde{\vx})$. To do so, CNCE models
$$p_{X,\tilde{X}|Y}(\vx,\tilde{\vx}|y)=p_{\tilde{X}|X}(\tilde{\vx}|\vx)p_X(\vx)1_{\{y=1\}}+p_{\tilde{X}|X}(\vx|\tilde{\vx})p_X(\tilde{\vx})1_{\{y=0\}},$$
and employs \cref{eq:NCE} Bayes optimal classifier, $p_{X}\leftarrow \exp(f_{\theta})$, to obtain
\begin{align}
    p_{Y|X}(1|\vx)=\sigmoid\left(\log\frac{p_{\tilde{X}|X}(\tilde{\vx}|\vx)\exp(f_{\theta}(\vx))}{p_{\tilde{X}|X}(\vx|\tilde{\vx})\exp(f_{\theta}(\tilde{\vx}))\nu}\right)\stackrel{\mbox{\tiny (if $p_{\tilde{X}|X}$ sym.)}}{=}\sigmoid\left(f_{\theta}(\vx)- f_{\theta}(\tilde{\vx})\nu\right),\label{eq:CNCE}
\end{align}
used to optimize $\theta$ via \cref{eq:cross_entropy}.
A further tie between CNCE (\cref{eq:CNCE}) and SM (\cref{eq:SM}) was found in the case where $\tilde{X}|X=X+\xi \epsilon$ with $\epsilon>0$ and $\xi$ a vector of uncorrelated random variables of mean zero and variance one that are independent from $X$ and have a symmetric density.

Then an extension to consider learning a conditional model i.e. $p(\vz|\vx;\theta)=\frac{1}{Z(\vx,\theta)}\exp(f_{\theta}(\vx,\vz))$ is studied in \citet{ma2018noise} with two possible losses corresponding to rank and binary classifications. The binary is the same as NCE. The ranking one is different as it compares the positive to all negative via softmax. Given samples $\{(\vx^{(n)},\vz^{(n)}),n=1,\dots,N\}$ and a noise distribution $p_{\epsilon}$ for $\vz$ one has
\begin{align}
    \mathcal{L}(\vx,\vz)=\log\frac{\exp\left(f_{\theta}(\vx^{(n)},\vz^{(n)})\right)}{\exp\left(f_{\theta}(\vx^{(n)},\vz^{(n)})\right)+\sum_{k}\exp\left(f_{\theta}(\vx^{(n)},\vz^{(n,k)})-\log p_{\epsilon}(\vz^{(n,k)})+\log p_{\epsilon}(\vz^{(n)})\right)}.\label{eq:CNCE}
\end{align}
and use the estimate $\hat{p}_{Z|X}(\vz|\vx)=\frac{\exp(f_{\theta}(\vx,\vz))}{\sum_{\vz \in \sZ}\exp(f_{\theta}(\vx,\vz))}$ with $\sZ$ the $\vz$s from the dataset.




A more significant improvement of NCE was coined Telescoping density-Ratio Estimation (TRE) \citep{rhodes2020telescoping}. In fact, notice that NCE learns the ratio $p_X/p_{\epsilon}$ by discriminating samples from $p_X$ and samples from $p_{\epsilon}$. TRE proposes instead to solve many sub-classification tasks to improve convergence and training stability. Denoting $p_{X}$ by $p_{X_1}$ and $p_{\epsilon}$ by $p_{X_0}$, we now introduce $K-2$ additional distributions $p_{X_{k}},k=1/K,\dots,(K-1)/K$  to produce the TRE estimate
\begin{align}
    \frac{p_{X_1}}{p_{X_0}}=\prod_{k=0}^{K-1}\frac{p_{X_k}}{p_{X_{k+1}}},
\end{align}
The distributions $p_{X_k}$ are defined through a {\em Waymark creation} strategy e.g. $X_k=\sqrt{1-\alpha_k^2}X_0+\alpha_k X_1$ with $\alpha_k \in (0,1),\alpha_0=0,\alpha_1=1$. Each classification problem is solved by a different classifier possibly sharing weights with each other. 

The next evolution introduced by \citet{choi2022density} is to take the infinite limit $K \rightarrow \infty$ and is coined TRE-$\infty$. In this case, there are infinitely many infinitesimal classification problems to solve. Hence instead of having to define some $p_{X_k}$, we only need to be able to sample continuously from it e.g. $X_k=\sqrt{1-\alpha(k)^2}X_0+\alpha(k) X_1$ where $\alpha$ is now a continuous function. Additionally, instead of having $K$ classifiers, we now have a single one with the time $t$ variable as input $f_{\theta}(\vx,t)$. This led to the creation of the time-score matching function 
\begin{align}
    \mathcal{L}_{TSM} = \mathbb{E}_{t \sim T}\left[\mathbb{E}_{\vx \sim X}\left[\frac{1}{2}\left\|f_{\theta}(\vx,t) -\frac{\partial\log(p_{X_t})}{\partial t}(\vx)\right\|_2^2\right]\right]
\end{align}


infinite limit  turns the classification problem into learning time scores (back to SM).

\begin{theorem}
Diffusion models correspond to doing infinitesimal NCE with joint matching and a RBF kernel density estimation.
\end{theorem}


However, $r(x)$ is unbounded and thus can take extremely large values when the denominator takes a small value. This causes robustness and stability issues \citep{liu2017trimmed}. To deal with this problem, a relative density-ratio has been proposed \citep{yamada2013relative}. For $\alpha \in [0,1)$, the relative density-
ratio $r_{\alpha}(\vx)$ is defined by 
\begin{align*}
    r_{\alpha}(\vx)=\frac{p_{X}(\vx)}{(1-\alpha)p_{\epsilon}(\vx)+\alpha p_{X}(\vx)},
\end{align*}


PU Learning \citep{du2015convex}
\begin{align*}
    \mathcal{L} = \pi \mathbb{E}_{p}[\ell(f(\vx),1)]-\pi\mathbb{E}_{p}[\ell(f(\vx),-1)]+\mathbb{E}_{u}[\ell(f(\vx),-1)],
\end{align*}
where $\ell$ is the logloss i.e. $\ell(f(\vx),1)=-\log(f(\vx))$ and $\ell(f(\vx),-1)=-\log(1-f(\vx))$ with $f: \mathcal{X} \mapsto [\epsilon,1-\epsilon]$. In this case the loss becomes
\begin{align*}
    \mathcal{L} = -\pi \mathbb{E}_{p}[\log(f(\vx))]+\pi\mathbb{E}_{p}[\log(1-f(\vx))]-\mathbb{E}_{u}[\log(1-f(\vx))].
\end{align*}
But then \citep{kiryo2017positive} found that this is not good with neural network cause overfitting and thus instead use
\begin{align*}
    \mathcal{L} = -\pi \mathbb{E}_{p}[\log(f(\vx))]+ReLU\left(\pi\mathbb{E}_{p}[\log(1-f(\vx))]-\mathbb{E}_{u}[\log(1-f(\vx))]\right).
\end{align*}

PU learning \citep{kato2018learning} with a selection bias i.e. $p(\vx|y=1,o=1) \not = p(\vx|y=1)$ minimizing the cost function from 



with kernel mean embedding \citep{ton2021noise}

sharing between samples, meta learning \citep{kumagai2021meta}

big review \url{https://project-archive.inf.ed.ac.uk/msc/20182768/msc_proj.pdf}

robust loss function under label noise \url{https://arxiv.org/pdf/1712.09482.pdf}

sampling \url{https://arxiv.org/pdf/1803.00942.pdf}

{\bf DRE For KL Estimation in Expectation-Maximization}
DRE used in EM  \citep{mescheder2017adversarial}. basically, the maximum likelihood is equal to the maximum log-likelihood since the log is a strictly increasing function i.e. 
\begin{align*}
    \log(u)<\log(u') \iff u<u',
\end{align*}
hence it is common to maximize the log-likelihood and its lower bound in the presence of unobserved variables $\vz$ as in
\begin{align*}
    \mathbb{E}_{\vx \sim X}\log(p_{X}(\vx_n;\theta))=&\mathbb{E}_{\vx \sim X}\log\left(\int p_{X|Z}(\vx_n|\vz;\theta)p_{Z}(\vz)d\vz\right)\\
    =&\mathbb{E}_{\vx \sim X}\log\left(\mathbb{E}_{\vz \sim (Z|X=\vx_n)}\left[\frac{ p_{X|Z}(\vx_n|\vz;\theta)p_{Z}(\vz)}{p_{Z|X}(\vz|\vx_n;\gamma)}\right]\right)\\
    \geq & \mathbb{E}_{\vx \sim X}\mathbb{E}_{\vz \sim (Z|X=\vx_n)}\left[\log\left(p_{X|Z}(\vx_n|\vz;\theta)\right)\right]-KL_{Z}\left(p_{Z|X}(\vz|\vx_n;\gamma)||p_{Z}(\vz)\right),
\end{align*}
however the KL term is nothing else but the ratio of probability between the posterior and prior. Hence whenever a closed-form solution is not available, this term can be approximated with any of the above techniques e.g. by training a discriminator with parameter $\eta$ to differentiate between the two distributions. Hence trianing involves updating $\eta$ for the discriminator to produce a correct estimate, and then learning $\theta,\gamma$ as usual i.e.
\begin{align*}
    \eta^* = \max \mathbb{E}_{\vx \sim X}\mathbb{E}_{\vz \sim (Z|\vx;\gamma)}+\mathbb{E}_{\vx \sim X}\mathbb{E}_{\vz \sim Z}+ \sigmoid(1-D(\vx,\vz)),\\
    (\theta^*,\gamma^*)=\max_{\theta,\gamma}\mathbb{E}_{\vx \sim X}\mathbb{E}_{\vz \sim (Z|X=\vx_n)}\left[\log\left(p_{X|Z}(\vx_n|\vz;\theta)\right)-D_{\eta^*}(\vx,\vz)\right],
\end{align*}
where in the last term gradient descent can be used easily, and no backpropagation is needed through $D$ because



Then \citep{takahashi2019variational} considered a different setting where the posterior is a simple distribution e.g. Gaussian but the prior is complicated. Hence it is the opposite as the above. In this case, the DRE can be done without $\vx$ as follows


extended it so that the discriminator does not depend on $\vx$ which simplifies the classification task.

Also learning a better prior in \citet{aneja2020ncp} modeled as a simple prior and a reweighting function so that only only needs to learn the ratio of the two, done through NCE.

hard negative sampling theory \citep{zhang2021understanding}

good review plus modeling of noise in labels \cite{gustafsson2020train}

library of reference in \url{https://github.com/yataobian/awesome-ebm}

likelihood and score based function \citep{song2021maximum}
